Quantum nuclear dynamics on a distributed set of ion-trap quantum computing systems

Quantum nuclear dynamics with wavepacket time-evolution is classically intractable and viewed as a promising avenue for quantum information processing. Here, we use an IonQ 11-qubit trapped-ion quantum computer, Harmony, to study the quantum wavepacket dynamics of a shared-proton within a short-strong hydrogen-bonded system. We also provide the first application of distributed quantum computing for chemical dynamics problems, where the distributed set of quantum processes is constructed using a tensor network formalism. For a range of initial states, we experimentally drive the ion-trap system to emulate the quantum nuclear wavepacket as it evolves along the potential surface generated from electronic structure. Following the experimental creation of the nuclear wavepacket, we extract measurement observables such as its time-dependent spatial projection and its characteristic vibrational frequencies to good agreement with classical results. Vibrational eigenenergies obtained from quantum computational are in agreement with those obtained from classical simulations to within a fraction of a kcal/mol, thus suggesting chemical accuracy. Our approach opens a new paradigm for studying the quantum chemical dynamics and vibrational spectra of molecules and also provides the first demonstration for parallel quantum computation on a distributed set of ion-trap quantum computers.

==> Figures_ionq/Fig_TN-trotter.tex <==
% Color palette
\definecolor{bblue}{rgb}{0.19, 0.55, 0.91}
\definecolor{green}{rgb}{0.0, 0.65, 0.58}
\definecolor{purple}{rgb}{0.6, 0.4, 0.8}
\definecolor{orange}{rgb}{0.83, 0.4, 0.32}

\begin{figure}[t!]
    \centering
    
    \tikzstyle{psi} = [rectangle, very thick, minimum width=4cm, minimum height = 0.7cm, inner sep=0.1cm,draw=purple, fill=purple!20]
    
    \tikzstyle{phi} = [circle, very thick, minimum size=1cm, inner sep=0.2mm, draw=orange, fill=orange!20]
    
    \tikzstyle{phinew} = [circle, very thick, minimum size=1cm, inner sep=0.2mm, draw=bblue, fill=bblue!20]
    
    % Time-Evolution operator tensor cores
    \tikzstyle{U} = [rectangle, very thick, minimum size=0.8cm, inner sep=0.1cm,draw=green, fill=green!20]
    
    % Define arrow style
    \tikzset{arw/.style={-Stealth, thick}}

    \begin{tikzpicture}[>=latex,node distance=3cm,
        every edge quote/.style={font=\fontsize{7}{1}},
        ]
        \node (psi1) [psi,font=\fontsize{9}{1}]{$\psi(x,\theta)$};
      
        \node (psix01) [below=0mm of psi1, xshift = -15mm, minimum size=0mm, inner sep=0mm]{};
        \node (psix02) [below=0mm of psi1, xshift = +15mm, minimum size=0mm, inner sep=0mm]{};

        \node (psix00) [below=2mm of psi1, minimum size=0mm, inner sep=0mm]{};
        
        \node (psix1) [below=2mm of psi1, xshift = -15mm, minimum size=0mm, inner sep=0mm]{};
        \node (psix2) [below=2mm of psi1, xshift = +15mm, minimum size=0mm, inner sep=0mm]{};
        
		\node (pphi1) [phi,below=8mm of psi1, xshift = -15mm, font=\fontsize{8}{1}]{$\phi_{1}(x)$};
        \node (pphi2) [phi, right=20mm of pphi1, font=\fontsize{8}{1}]{$\phi_{2}(\theta)$};

        \node (ppx01) [below=6mm of psix00, minimum size=0mm, inner sep=0mm]{}; 
        
        \node (ppx1) [below=2mm of pphi1, minimum size=0mm, inner sep=0mm]{};
        \node (ppx2) [below=2mm of pphi2, minimum size=0mm, inner sep=0mm]{};
        
        \node (V1) [U, below=2mm of ppx1, font=\fontsize{8}{1}]{$\mathcal{V}_{1}$};
        \node (V2) [U, below=2mm of ppx2, font=\fontsize{8}{1}]{$\mathcal{V}_{2}$};
                
        \node (K1) [U, below=2mm of V1, font=\fontsize{8}{1}]{$\mathcal{K}_{1}$};
        \node (K2) [U, below=2mm of V2, font=\fontsize{8}{1}]{$\mathcal{K}_{2}$};
         

        \node (u1) [U, below=2mm of K1, font=\fontsize{8}{1}]{$\mathcal{V}_{1}$};
        \node (u2) [U, below=2mm of K2, font=\fontsize{8}{1}]{$\mathcal{V}_{2}$};
             
        \node (ux1) [below=3mm of u1, minimum size=0mm, inner sep=0mm]{};
        \node (ux2) [below=3mm of u2, minimum size=0mm, inner sep=0mm]{};
        
        \node (eql0sgn) [below=10mm of ux1, right=13mm of ux1]{};
        \node (eqlsgn) [below=5mm of eql0sgn]{};  
        
        \node (phit1) [phinew, below=12mm of u1, font=\fontsize{8}{1}]{$\varphi_{1}(x)$};
        \node (phit2) [phinew, below=12mm of u2, font=\fontsize{8}{1}]{$\varphi_{2}(\theta)$};
        
        \node (phitx1) [below=3mm of phit1, minimum size=0mm, inner sep=0mm]{};
        \node (phitx2) [below=3mm of phit2, minimum size=0mm, inner sep=0mm]{};
        

        \draw[-To, very thick, black, to path={-| (\tikztotarget)}] (eql0sgn) edge (eqlsgn);
        \draw[-To, very thick, black, to path={-| (\tikztotarget)}] (psix00) -- (ppx01);
        
        \path[-]
            
%           \draw[arw,thick,draw=black] (eql0sgn.south) -| (eqlsgn.north);
           
%            (eql0sgn) edge[very thick, purple] (eqlsgn)
            (psix01) edge[very thick, purple] node[left,black, yshift=-1mm, font=\fontsize{10}{1}] {} (psix1)
            (psix02) edge[very thick, purple] 
            node[left,black, yshift=-1mm,font=\fontsize{10}{1}] {} (psix2)

%            (psix00) edge[thick, black] 
%            node[left,black, yshift=-1mm,font=\fontsize{10}{1}] {} (ppx01)
%            (psix00) edge[thick, black] 
%           node[left,black, yshift=-1mm,font=\fontsize{10}{1}] {} (ppx02)
            
            (pphi1) edge[very thick, orange] node[above,black,font=\fontsize{10}{1}] {} (pphi2)
           
            (pphi1) edge[very thick, orange] node[left,black,yshift=-1mm,font=\fontsize{10}{1}] {} (ppx1)
            (pphi2) edge[very thick, orange] node[left,black,yshift=-1mm,font=\fontsize{10}{1}] {} (ppx2)
            
            (V1) edge[very thick, green] node[above,black,font=\fontsize{10}{1}] {} (V2)
            
            (u1) edge[very thick, green] node[below,black,font=\fontsize{10}{1}] {} (u2)
            

            (V1) edge[very thick, green] (ppx1)
            (u1) edge[very thick, green] node[left,black,yshift=-0.5mm,font=\fontsize{10}{1}] {}(ux1)
            (V2) edge[very thick, green] (ppx2)
            (u2) edge[very thick, green] node[left,black,yshift=-0.5mm,font=\fontsize{10}{1}] {}(ux2)
            
            (V1) edge[very thick, green] (K1)
            (V2) edge[very thick, green] (K2)

            (u1) edge[very thick, green] (K1)
            (u2) edge[very thick, green] (K2)

            (phit1) edge[very thick , bblue] node[above,black,font=\fontsize{10}{1}] {} node[below,black] {} 
            (phit2)
           
            (phit1) edge[very thick, bblue] node[left,black,yshift=-0.5mm,font=\fontsize{10}{1}] {}(phitx1)
            (phit2) edge[very thick, bblue] node[left,black,yshift=-0.5mm,font=\fontsize{10}{1}] {}(phitx2)
            ;

           
    \end{tikzpicture}

    \caption{The figure shows the action of the time evolution operator onto the wave function. The unitary operator in Eq. \ref{Eq:Trotter} is decomposed here into one-dimensional kinetic and potential propagators.}
    \label{Fig:MPS_tEvo_trotter}
\end{figure}
